Generative Interest Estimation for Document Recommendations

Learning distributed representations of documents has pushed the state-of-the-art in several natural language processing tasks and was successfully applied to the field of recommender systems recently. In this paper, we propose a novel content-based recommender system based on learned representations and a generative model of user interest. Our method works as follows: First, we learn representations on a corpus of text documents. Then, we capture a user's interest as a generative model in the space of the document representations. In particular, we model the distribution of interest for each user as a Gaussian mixture model (GMM). Recommendations can be obtained directly by sampling from a user's generative model. Using Latent semantic analysis (LSA) as comparison, we compute and explore document representations on the Delicious bookmarks dataset, a standard benchmark for recommender systems. We then perform density estimation in both spaces and show that learned representations outperform LSA in terms of predictive performance.

==> Makefile <==
engine = "pdflatex -interaction=nonstopmode --shell-escape %O %S"
refs = references.bib
sources = main.tex $(wildcard section/*.tex)
output = 'output'

main.pdf: $(sources)
	@latexmk -pdf -pdflatex=${engine} -output-directory='$(output)' -bibtex $<

watch:
	@while ! inotifywait --event modify $(refs) $(sources); do make; done

spell:
	@hunspell -l -t -d en_US -i utf-8 $(sources) \
		| sort \
		| uniq --ignore-case \
		| grep -vxFf dictionary.txt

clean:
	@latexmk -C
	rm -rf $(output)/*

pack:
	cp output/main.bbl .
	tar -czvf ../genrec.tar --exclude .git --exclude output .

.PHONY: watch spell clean

